Concurrent Scheduling of Event-B Models

Event-B is a refinement-based formal method that has been shown to be useful in developing concurrent and distributed programs. Large models can be decomposed into sub-models that can be refined semi-independently and executed in parallel. In this paper, we show how to introduce explicit control flow for the concurrent sub-models in the form of event schedules. We explore how schedules can be designed so that their application results in a correctness-preserving refinement step. For practical application, two patterns for schedule introduction are provided, together with their associated proof obligations. We demonstrate our method by applying it on the dining philosophers problem.

==> eptcsdata.tex <==
\providecommand{\firstpage}{166}
\providecommand{\publicationstatus}{J. Derrick , E.A. Boiten, S. Reeves (Eds.):\\
Refinement Workshop 2011.
\\
EPTCS 55, 2011, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.55.11}{10.4204/EPTCS.55.11}}

